BP-NTT: Fast and Compact in-SRAM Number Theoretic Transform with Bit-Parallel Modular Multiplication

Number Theoretic Transform (NTT) is an essential mathematical tool for computing polynomial multiplication in promising lattice-based cryptography. However, costly division operations and complex data dependencies make efficient and flexible hardware design to be challenging, especially on resource-constrained edge devices. Existing approaches either focus on only limited parameter settings or impose substantial hardware overhead. In this paper, we introduce a hardware-algorithm methodology to efficiently accelerate NTT in various settings using in-cache computing. By leveraging an optimized bit-parallel modular multiplication and introducing costless shift operations, our proposed solution provides up to 29x higher throughput-per-area and 2.8-100x better throughput-per-area-per-joule compared to the state-of-the-art.

==> Elaheh_notes.tex <==
Highlight
-Re-purposing Cache, add more relevant data for the integration

Todos 
-Run the Grammarly 
- Where each of these benefits are coming from 


Discuss: 
-What are the related work
-What is the main issue with the related work? 
-How we are addressing it? 
- comparing with neural cache, that is based on the bit-serial desing? 
 
 
